RealProbe: An Automated and Lightweight Performance Profiler for In-FPGA Execution of High-Level Synthesis Designs

High-level synthesis (HLS) accelerates FPGA design by rapidly generating diverse implementations using optimization directives. However, even with cycle-accurate C/RTL co-simulation, the reported clock cycles often differ significantly from actual FPGA performance. This discrepancy hampers accurate bottleneck identification, leading to suboptimal design choices. Existing in-FPGA profiling tools, such as the Integrated Logic Analyzer (ILA), require tedious inspection of HLS-generated RTL and manual signal monitoring, reducing productivity. To address these challenges, we introduce RealProbe, the first fully automated, lightweight in-FPGA profiling tool for HLS designs. With a single directive--#pragma HLS RealProbe--the tool automatically generates all necessary code to profile cycle counts across the full function hierarchy, including submodules and loops. RealProbe extracts, records, and visualizes cycle counts with high precision, providing actionable insights into on-board performance. RealProbe is non-intrusive, implemented as independent logic to ensure minimal impact on kernel functionality or timing. It also supports automated design space exploration (DSE), optimizing resource allocation based on FPGA constraints and module complexity. By leveraging incremental synthesis and implementation, DSE runs independently of the original HLS kernel. Evaluated across 28 diverse test cases, including a large-scale design, RealProbe achieves 100% accuracy in capturing cycle counts with minimal logic overhead-just 16.98% LUTs, 43.15% FFs, and 0% BRAM usage. The tool, with full documentation and examples, is available on GitHub at https://github.com/sharc-lab/RealProbe .

==> figs/fig_bumponly.tex <==
\begin{figure}[ht!]
    % \includegraphics[trim={1cm 8cm 9cm 1cm},clip,width=7.5in]{./figs/bottleneck.pdf}
    % \includegraphics[trim={0.1cm 20.5cm 4.7cm 0.1cm},clip,width=7.5in]{./figs/bottleneck_test.pdf}
    \includegraphics[trim={0.1cm 0.1cm 2.5cm 0.1cm},clip,width=3.55in]{./figs/bumpchart.pdf}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Function execution timelines and bottleneck analysis by cycle count ranking across C-synth, Co-sim, and RealProbe}
    \label{fig_bump}
\end{figure}

==> figs/fig_comp.tex <==
\begin{figure}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[trim={0.1cm 0.05cm 0.1cm 0.1cm},clip,width=3.55in]{./figs/comp.pdf}
    \caption{Runtime comparison between original design, original design with RealProbe, and original design with ILA.}
    \label{fig_system} 
\end{figure}

==> figs/fig_maxfreq.tex <==
\begin{figure}
%\vspace{-12pt}
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{-12pt}
    \includegraphics[trim={0.1cm 0.1cm 0.1cm 0.1cm},clip,width=3.55in]{./figs/maxfreq.pdf}
    \caption{\textcolor{rev}{Impact of RealProbe integration on maximum frequency of the original design.}}
    \label{fig_maxfreq} 
    \vspace{-0pt}
\end{figure}

==> figs/fig_pragmacode.tex <==
\begin{figure}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{-10pt}
    \includegraphics[trim={0.5cm 41cm 10.5cm 0.4cm},clip,width=3.55in]{./figs/pragmacode.pdf}
    \caption{Code snippet of the modified Clang/LLVM to support RealProbe and the generated LLVM IR}
    \label{fig_pragmacode}
\end{figure}

==> tbls/tbl_diff.tex <==

\begin{table}[!bt]
    \setlength{\tabcolsep}{4pt}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{5pt}
    \footnotesize   
    \renewcommand{\arraystretch}{\myarraystretch}
    \begin{threeparttable}
    
    \caption{Descripencies between C/RTL co-sim and on-board performance measured in latency under 100 MHz clock frequency. Results are on Pynq-Z2 FPGA evaluation board.}
    \label{tbl_report}
    \begin{tabular}{c|c|c|c|c} 
    \toprule

    Benchmark & Version & C-synth & Co-sim & On-board \\ \midrule
    Matrix & Unoptimized & 32 ms & 32.5 ms & 53.05 ms \\ %\hline
     Multiplication & Array partition & 3.29 ms & 3.42 ms & 6.04 ms \\ %\hline
     & 1D loop tiling & 1.10 ms & 1.13 ms & 3.25 ms \\ %\hline
     & 2D loop tiling & 0.65 ms & 0.685 ms & 1.94 ms \\ \hline

     Apply  & Unoptimized & 5.368 ms & 5.368 ms & 9.77 ms \\ %\hline

     Watermark & Loop unroll (16-bit) & 0.317 ms & 0.357 ms & 5.19 ms \\ %\hline

     & Loop unroll (32-bit) & 0.317 ms & 0.357 ms & 5.48 ms \\ %\hline

     & Streaming (16-bit) & 0.317 ms & 0.357 ms & 5.19 ms \\ %\hline

     & Streaming (32-bit) & 0.317 ms & 0.357 ms & 5.21 ms \\ \hline

     \ch{more if any} & \\

    \bottomrule
    
    \end{tabular}\label{tbl_diff}

    % \begin{tablenotes}
    %     \item[a] C-sim results are extracted in C-sim code analyzer reports
    %     \item[b] This is not provided by Vitis HLS, but user can measure the time manually
    % \end{tablenotes}
\end{threeparttable}
    
\end{table}

==> tbls/tbl_impact.tex <==
\begin{table*}[ht]
\vspace{-12pt}
    \centering
    \scriptsize
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{5pt}
    \setlength{\tabcolsep}{4.5pt}
    \renewcommand{\arraystretch}{\myarraystretch}
    \begin{threeparttable}
    \caption{Impact of different function inline options and incremental synthesis.}
    \label{tbl_impact}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \hline \hline
    \multirow{2}{*}{Benchmark} & \multirow{2}{*}{Design} & \multicolumn{3}{c|}{Resource Usage} & \multicolumn{3}{c|}{Run time} & \multirow{2}{*}{WNS (ns)} & \multirow{2}{*}{Fmax (Mhz)} \\ \cline{ 3- 8} 
    &&\textbf{LUTs} & \textbf{FFs} & \textbf{BRAMs} & \textbf{C-synth (s)} & \textbf{Vivado (s)} & \textbf{On-FPGA (us)} &  \\ \hline\hline
    \multirow{4}{*}{\tworows{Nested}{function}}        & Original        & 3768          & 6448          & 1                      & 17           &  261        & 117.98                       & 0.152   & 101.54                                                        \\ \cline{ 2- 10}
                       & RealProbe w/ inline\_off\_top       & 3985 (+5.76\%)          & 6890 (+6.85\%)         & 1                   & 18                     & 245                           & 111.24                       &      0.259               &   102.66      \\ \cline{ 2- 10}
                       & RealProbe w/ inline\_off\_all       & 4605 (+22.21\%)         & 7514 (+16.53\%)          & 1                   & 18                    & 262                           & 102.09                   &         0.352              &    103.65   \\ \cline{ 2- 10}
                       & RealProbe w/ function update       & 4174 (+10.77\%)          & 7062 (+9.52\%)         & 1                   & 0                     & 51                           & 104.52                    &          0.298            &  103.07     \\ \hline\hline
    \end{tabular}   
    \end{threeparttable}
    \end{table*}
    

==> tbls/tbl_incremental.tex <==
\begin{table}[!bt]
\vspace{-12pt}
    \setlength{\tabcolsep}{4.8pt}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{5pt}
    \footnotesize   
    \renewcommand{\arraystretch}{\myarraystretch}
    \begin{threeparttable}
    
    \caption{Total cycle count of Matrix multiplication with different targeting FPGA board, different optimization directives, different synthesis and implementation strategies}
    \begin{tabular}{c|c|c|c} 
    % \toprule
    \hline
           & Reference run   & Incremental synthesis    & Incremental implementation\\ \hline

    &&& \\\hline
    &&& \\\hline
    (P) w/ array part. & 34849 (-1.2\%) & 35047 (-0.6\%) & 35270 \\\hline
    (P) w/ unroll & 34849 (-1.2\%) & 35047 (-0.7\%) & 35281 \\\hline
    (P) w/ DRAM & 631873 (-65.9\%) & 1069174 (-42.2\%) & 1850604 \\\hline
    (P) w/ flow opt. & 168025 (-0.3\%) & 168229 (-0.1\%) & 168457 \\\hline
    (P) w/ perf opt. & 168025 (-0.3\%) & 168229 (-0.1\%) & 168460 \\\hline
    (P) w/ area opt. & 168025 (-0.3\%) & 168229 (-0.1\%) & 168448 \\\hline\hline
    ZCU102 board (Z) & 69721 (-0.4\%) & 69922 (-0.1\%) & 69984 \\\hline
    (Z) w/ DRAM & 566337 (-79.7\%) & 1069174 (-61.6\%) & 2787078 \\\hline
    
    \end{tabular}\label{tbl_gemm}
    
\end{threeparttable}
    
\end{table}

==> tbls/tbl_refs.tex <==
\begin{table}[!bt]
\vspace{-12pt}
\usepackage[font=small, skip=4pt]{caption}

    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{-10pt}
    \setlength{\tabcolsep}{4.8pt}
    \footnotesize   
    \renewcommand{\arraystretch}{\myarraystretch}
    \begin{threeparttable}
    
    \caption{Total cycle count of Matrix multiplication with different targeting FPGA board, different optimization directives, different synthesis and implementation strategies}
    \begin{tabular}{c|c|c|c} 
    \toprule
    \hline
    Version       & C-synth   & Co-sim    & RealProbe\\ \hline\hline

    Pynqz2 board (P) & 168025 (-0.3\%) & 168229 (-0.1\%) & 168449 \\\hline
    (P) w/ pipeline & 34847 (-1.2\%) & 35047 (-0.6\%) & 35271 \\\hline
    (P) w/ array part. & 34849 (-1.2\%) & 35047 (-0.6\%) & 35270 \\\hline
    (P) w/ unroll & 34849 (-1.2\%) & 35047 (-0.7\%) & 35281 \\\hline
    (P) w/ DRAM & 631873 (-65.9\%) & 1069174 (-42.2\%) & 1850604 \\\hline
    (P) w/ flow opt. & 168025 (-0.3\%) & 168229 (-0.1\%) & 168457 \\\hline
    (P) w/ perf opt. & 168025 (-0.3\%) & 168229 (-0.1\%) & 168460 \\\hline
    (P) w/ area opt. & 168025 (-0.3\%) & 168229 (-0.1\%) & 168448 \\\hline\hline
    ZCU102 board (Z) & 69721 (-0.4\%) & 69922 (-0.1\%) & 69984 \\\hline
    (Z) w/ DRAM & 566337 (-79.7\%) & 1069174 (-61.6\%) & 2787078 \\\hline
    \bottomrule
    
    \end{tabular}\label{tbl_gemm}
    
\end{threeparttable}

\end{table}
